Understanding and Improving Transfer Learning of Deep Models via Neural Collapse

With the ever-increasing complexity of large-scale pre-trained models coupled with a shortage of labeled data for downstream training, transfer learning has become the primary approach in many fields, including natural language processing, computer vision, and multi-modal learning. Despite recent progress, the fine-tuning process for large-scale pre-trained models in vision still mostly relies on trial and error. This work investigates the relationship between neural collapse (NC) and transfer learning for classification problems. NC is an intriguing while prevalent phenomenon that has been recently discovered in terms of the final-layer features and linear classifiers of trained neural networks. Specifically, during the terminal phase of training, NC implies that the variability of the features within each class diminishes to zero, while the means of features between classes are maximally and equally distanced. In this work, we examine the NC attributes of pre-trained models on both downstream and source data for transfer learning, and we find strong correlation between feature collapse and downstream performance. In particular, we discovered a systematic pattern that emerges when linear probing pre-trained models on downstream training data: the more feature collapse of pre-trained models on downstream training data, the higher the transfer accuracy. Additionally, we also studied the relationship between NC and transfer accuracy on the source data. Moreover, these findings allow us to develop a principled, parameter-efficient fine-tuning method that employs skip-connection to induce the last-layer feature collapse on downstream data. Our proposed fine-tuning methods deliver good performances while reducing fine-tuning parameters by at least 90% and mitigating overfitting in situations especially when the downstream data is scarce.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Added 
\newcommand{\NC}{$\mathcal {NC}$}
\newcommand{\mb}{\bm}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mrm}{\mathrm}
\newcommand{\mtt}{\mathtt}
\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }
\newcommand{\wh}{\widehat}
\newcommand{\wc}{\widecheck}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\rank}{\operatorname{rank}}
% Added done

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/exp-layerwise_qing.tex <==

Finally, we compliment our study by examining the relationship between the \NC\ metrics and transfer accuracy on the source training dataset. Compared to recent studies on the relationship between feature diversity and transfer accuracy \cite{islam2021broad,kornblith2021why}, our work not only examines the effect of different training losses  but also (\emph{i}) provides insights into several popular heuristics in model pre-training (e.g. projection head, data augmentation), and (\emph{ii}) reveals the limitations of using feature diversity as the sole metric for evaluating the quality of pre-trained models. Specifically, we show that the positive correlation between feature diversity on source data (indicated by larger \NC$_1$) and transfer accuracy only holds within a certain extent.\footnote{This positive correlation only holds up to a certain extent as random features do not collapse, but they do not generalize well. This is because random features are not discriminative. We conjecture that there could be a trade-off between feature diversity and discrimination.} %we find that the two are positively correlated, meaning that larger \NC\ metrics lead to better transfer accuracy, echoing recent findings in \cite{islam2021broad,kornblith2021why}. The reasoning is that if the learned representations are less collapsed on the pre-training data, they better preserve the intrinsic structures of the inputs. Furthermore, 

%We begin our investigation by studying the relationship between \NC\ metrics and transfer accuracy on \emph{pre-training dataset}. Within a certain range,\footnote{As random features do not collapse but not generalize well, the positive correlation above only holds to a certain extent. The reason is that random features are not discriminative. We conjecture that there could be a trade-off between feature diversity and discrimination.} we show that the two are positively correlated -- larger \NC\ metrics lead to better transfer accuracy, which echoes recent discoveries in \cite{islam2021broad,kornblith2021why}. The intuition is that if the learned representations are less collapsed on the pre-training data, they better preserve the intrinsic structures of the inputs. Moreover, compared to \cite{islam2021broad,kornblith2021why}, our work not only studies the effect of different training losses on feature diversity, but also (\emph{i}) provides insights for several heuristics in model pre-training (e.g., projection head, data augmentation), and (\emph{ii}) reveals the limitations of using feature diversity as the only metric for evaluating representation quality of pre-trained models.

\paragraph{Impact of training losses and network architectures on feature diversity and transferability.} Our investigation shows that the choice of training losses and the design of network architecture have a substantial impact on the levels of feature collapse on the penultimate layer and hence on the transfer accuracy. Similar observations were made in \cite{islam2021broad,kornblith2021why} regarding the impact of different training losses on transfer performance. To demonstrate this, we pre-trained ResNet18 models on the Cifar-100 dataset using three different loss functions: CE, MSE \citep{hui2020evaluation}, and SupCon \citep{khosla2020supervised}. We then evaluated the test accuracy on the Cifar-10 dataset by training a linear classifier on the frozen pre-trained models. For the SupCon loss, we followed the setup described in \cite{khosla2020supervised}, which uses an MLP as a projection head after the ResNet18 encoder. However, after pre-training, we only used the encoder network as the pre-trained model for downstream tasks and abandoned the projection head. The results of $\mathcal{NC}_1$ and the corresponding transfer accuracy for each scenario are summarized in \Cref{tab:initial_exp}, where the last two columns reports the results for SupCon with different layers of projection heads. From \Cref{tab:initial_exp}, we observe the following.

%\paragraph{Choices of training losses and architectures impact feature diversity and hence transferability.} First, we show that the choice of training losses and design of architecture substantially affects the levels of feature collapse on the penultimate layer and the transfer accuracy.\footnote{For the choices of loss, the works \cite{islam2021broad,kornblith2021why} have similar observations, where different choices of training losses for pre-training lead to different transfer performance.} To experimentally demonstrate this, we pre-train ResNet18 models on the Cifar-100 dataset with three different choices of loss functions: CE, MSE \cite{hui2020evaluation}, and SupCon \cite{khosla2020supervised}). Once the models are trained, we evaluate the test accuracy on the Cifar-10 dataset, by only learning a linear classifier upon the frozen pre-trained models. In \Cref{tab:initial_exp}, we summarize the results of $\mathcal{NC}_1$ on all pre-trained models and the corresponding transfer accuracy under different training scenarios. For the SupCon loss, we follow the original setup in \cite{khosla2020supervised} that uses a nonlinear multi-layer perception (MLP) module as a projection head after the ResNet18 encoder; once the model has been pre-trained, we only use the encoder network as the pre-trained model for downstream tasks with the projection head abandoned. The results of SupCon with different projection heads are reported in the last two columns of \Cref{tab:initial_exp}. As we observe from \Cref{tab:initial_exp}, 
\begin{itemize}[leftmargin=*]
    \vspace{-0.1in}
    \item \emph{The choice of training loss impacts feature diversity, which in turn affects transfer accuracy.} Larger feature diversity, as measured by a larger \NC$_1$ value, generally leads to better transfer accuracy. For example, a model pre-trained with the MSE loss exhibits a severely collapsed representation on the source dataset, with the smallest \NC$_1$ value and the worst transfer accuracy.
    \vspace{-0.1in}
    \item \emph{The MLP projection head is crucial for improved transferability.} The model pre-trained with the SupCon loss and a multi-layer MLP projection head shows the least feature collapse compared to the other models and demonstrates superior transfer accuracy.\footnote{This observation aligns with recent work \citep{islam2021broad}.} If we substitute the MLP with a linear projection layer, both the \NC$_1$ metric and transfer accuracy of SupCon decrease, resulting in performance comparable to the models pre-trained with the CE loss.
\end{itemize}
Building on the above observation, in the following we delve deeper into the role of the projection head in transfer learning by exploring the progressive decay of the $\mathcal{NC}_1$ metric across layers.
% On the other hand,   where SupCon leads to better transferability than CE. This is because SupCon with MLP projection layers learns more diverse features (larger \NC$_1$) than CE. However, when no projection layer presents, it has been proven that both SupCon and CE should learn the same \NC\ representations under the so-called unconstrained features model assumption \cite{fang2021exploring,zhu2021geometric,graf2021dissecting}. This contradiction raises an interesting question on the effects of projection layers for transferability, that we further address in the following through the phenomenon of progressive \NC\ across layers.

%given both SupCon and CE learn the same \NC\ representations in the so-called unconstrained features model \cite{fang2021exploring,zhu2021geometric,graf2021dissecting}, it raises an interesting question on why the features learned by SupCon are more diverse. We further address this question in the following.

%why this is the case given that both SupCon and CE learn \NC\ representations in the so-called unconstrained features model \cite{fang2021exploring,zhu2021geometric,graf2021dissecting}?

 \begin{table}[t]
 \caption{\textbf{Comparisons of \NC$_1$ and transfer accuracy with different training losses and settings.} We pre-train ResNet18 models on the Cifar-100 dataset, and then test the models on Cifar-10. We use proj. to denote projection head; w/o proj. means without projection head, w/linear proj. means adding one linear layer projection layer, and w/ mlp proj. means adding a two-layer MLP projection. }
\centering
\resizebox{\linewidth}{!}{
	\begin{tabular}	{c || c | c | c | c  } 
		\toprule	 	
		 \textbf{Training} & MSE (w/o proj.) & Cross-entropy (w/o proj.) & SupCon (w/ linear proj.)& SupCon (w/ mlp proj.) \\
		 
		 \midrule
		 \textbf{$\mathcal{NC}_1$ (Cifar-100)} & 0.001 & 0.771 & 0.792 & 2.991\\ 
		 \midrule
		 \textbf{Transfer Acc.} & 53.96 & 71.2 & 69.89 & 79.51 \\ 
	    \bottomrule
	\end{tabular}}
	
    
    \label{tab:initial_exp}
    % \vspace{-0.1in}
\end{table}

 \begin{figure}[t]
    \centering
    \includegraphics[width = 0.29\textwidth]{figs/C100_CE_NC1_proj.pdf}
    \hspace{0.08in}
    \includegraphics[width = 0.29\textwidth]{figs/C100_MSE_nc1_proj.pdf}
    \hspace{0.08in}
    \includegraphics[width = 0.29\textwidth]{figs/C100_SupCon_nc1_proj.pdf}
    \caption{\textbf{Trend of $\mc {NC}_1$ during training and transfer learning accuracy of the pretrained models.} ResNet-50 models are pretrained using Cifar-100 dataset with CE loss (Left), MSE loss (Middle) and SupCon loss (Right). Models are pretrained with different numbers of layers for projection heads and transfered on the Cifar-10 dataset.}
    \label{fig:ce_nc_transfer}
    \vspace{-0.1in}
\end{figure}
%\qq{The legend is not consistent, should be "two layers MLP" instead of "two layers"}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 0.35\textwidth]{figs/C100_MSE_nc1_proj.pdf}
%     \hspace{0.1in}
%     \includegraphics[width = 0.35\textwidth]{figs/C100_SupCon_nc1_proj.pdf}
%     \caption{\textbf{Trend of $\mc {NC}_1$ during training and transfer learning accuracy of the pretrained models.} ResNet50 models are pretrained using Cifar-100 dataset with MSE loss (Left) and SupCon (Right). Models are pretrained with different numbers of layers for projection heads and transfered on the Cifar-10 dataset. }
%     \label{fig:mse_supcon_proj}
% \end{figure}

%(However, we should not expect the transfer accuracy to be improved infinitely)
\begin{wrapfigure}[18]{R}{0.34\textwidth}
\vspace{-0.2in}
    \centering
    \includegraphics[width = 0.31\textwidth]{figs/alg_adv_nc_fail.pdf}
    \caption{\textbf{$\mc {NC}_1$ vs. transfer learning accuracy.} Models are pre-trained on the Cifar-100 dataset with different levels of data augmentation and adversarial training strength, and then transfer accuracy of pre-trained models is reported on the Cifar-10 dataset.}
    \label{fig:alg_adv_nc_fail}
\end{wrapfigure} 

\paragraph{Projection layers in pre-training increase feature diversity for better transferability.} 
The use of projection head for model pre-training was first introduced and then gained popularity in self-supervised learning \citep{chen2020simple,chen2021exploring}, but the reason for its effectiveness is not fully understood. On this end, previous work \citet{he2022law} has demonstrated that the feature within-class variability collapses progressively from shallow to deep layers, with the collapse becoming more severe in deeper layers (i.e., smaller $\mc {NC}_1$ values). Based upon this discovery, we conclude that the use of a projection layer in pre-training helps to prevent the variability collapse of the encoder network, thereby better preserving the information of the input data with improved transfer performance.

This can be demonstrated by our experiments in \Cref{fig:ce_nc_transfer}, where we pre-train ResNet-50 models on the Cifar-100 dataset and report \NC\ metrics and transfer accuracy for varying numbers of projection head layers (from one to three layers). Our results show that using projection heads significantly increases representation diversity and transfer accuracy -- adding more layers of MLP projection leads to higher \NC$_1$ and improved transfer accuracy, although the performance improvement quickly plateaus at three layers of MLP. This suggests that the effectiveness of projection heads in model pre-training is not limited to contrastive losses but applies universally across various training loss types (e.g. CE and MSE).

%This can be demonstrated by our experiments in \Cref{fig:ce_nc_transfer}, where we pre-train ResNet-50 models on the Cifar-100 dataset and report the \NC\ and transfer accuracy for a different number of layers of projection heads (from one to three layers). We show that the usage of projection heads substantially increases the diversity of the representations and the transfer accuracy -- more layers of MLP projection lead to larger \NC$_1$, and hence better transfer accuracy, although the performance gain quickly saturates upon three layers of MLP. Such an observation implies that the effectiveness of projection heads for model pre-training is nothing particular for contrastive losses, but is universal across different types of training losses (e.g., CE and MSE).


%This phenomenon is quite universal across different training losses (e.g., CE, MSE, and SupCon), where effectiveness of projection heads for model pre-training is not spe contrastive losses. 


% In \Cref{fig:ce_nc_transfer}, we can observe that the inclusion of pcompared with that of no projection head.



%We empirically verify this conjecture by replacing the MLP by a linear layer for the projection head in SupCon and then train the model under the same setting. We observe from \Cref{tab:initial_exp} that SupCon with a linear projection head indeed achieves similar \NC\ and transfer accuracy as CE.
%Note that the layer-wise progressive collapse is universal across the choice of training losses, the usage of projection head is not limited to contrastive losses. Thus, we can also improve the transferability for supervised pre-training models with the CE / MSE loss by adding a MLP projection head. To verify this, we pre-train ResNet-50 models (we use it for better performance) on the Cifar-100 dataset. We report the \NC\ and transfer accuracy for different choices of projection heads. %Thus, suggests that the usage of  projection haeds for improving transferability can be universal.
%We note that 
 

 

% \paragraph{Projection layers in pre-training increase feature diversity for better transferability.}
%  When training deep models, the outputs of encoder network are often not used directly. Rather, they are further passed though a nonlinear multi-layer perception (MLP) module $\mb g(\cdot)$, known as the projection head, to improve the representation quality. Once the model has been trained, the projection head will be abandoned and only the encoder network will be utilized for downstream tasks. Such a technique is first introduced for contrastive learning \cite{chen2020simple} and popularized for pre-training deep models \cite{khosla2020supervised,chen2021exploring}, while the reasons behind the success of such a method remain as mystery. Here, we demystify the underlying mechanism of projection head based upon progressive variability collapse, where our experiments show that the usage of projection heads is not limited to contrastive losses. 

%  \begin{table}[t]
% \centering
% \resizebox{0.75\linewidth}{!}{
% 	\begin{tabular}	{c || c | c | c  } 
% 		\toprule	 	
% 		 \textbf{Training} & MSE (w/o proj.) & Cross-entropy (w/o proj.) & SupCon (w/ proj.) \\
% 		 \midrule
% 		 \textbf{$\mathcal{NC}_1$ (Cifar-100)} & 0.015 & 0.195 & 0.688 \\ 
% 		 \midrule
% 		 \textbf{Transfer Acc.} & 57.02 & 64.29 & 78.55 \\ 
% 	    \bottomrule
% 	\end{tabular}}
	
%     \caption{\textbf{Transfer learning results \& model $\mathcal{NC}_1$ comparison among different training settings.} ResNet18 models are pre-trained on the Cifar-100 dataset and transfered on Cifar-10. All models are trained for $500$ epochs. We use proj. to denote projection head.}
%     \label{tab:initial_exp}
% \end{table}
 
%  In \Cref{tab:initial_exp}, we summarize the results of model $\mathcal{NC}_1$ and transfer accuracy for different training scenarios. As we can see, the model trained with the MSE loss \cite{hui2020evaluation} is severely collapsed on the source dataset and has a inferior transfer accuracy while the model trained using the supervised contrastive loss (SupCon) \cite{khosla2020supervised} with projection head is less collapse compared to the other models and has superior transfer performance. We conjecture that the inclusion of projection head serves as an important role of such advantage: due to layer-wise progressive collapse, the additional projection layers prevent severe variability collapse of the encoder network. Moreover, because the layer-wise progressive collapse is universal across the choice of training losses, the usage of projection head is not limited to contrastive losses nor self-supervised pre-training. To verify our conjecture, we add different layers of projection heads for supervised pre-training models with the CE loss and report the results for two different pre-training datasets (Cifar-100 and MiniImageNet) in \Cref{fig:ce_nc_transfer}. We can obseve that the inclusion of projection heads substantially increase the transfer accuracy compared with that of no projection head. This suggests that the usage of projection for improving transferability can be universal.
 
 % To verify our conjecture, we add different number of projection layers (i.e., 1-3 layers) for model pre-training. \Cref{fig:ce_nc_transfer} shows that more layers of projection head leads to better feature diversity of the encoder network, measured by $\mc {NC}_1$. Moreover,

%\paragraph{} 
\vspace{-0.1in}
\paragraph{Usage of the pre-trained \NC\ metric for predicting transfer accuracy has limitations.} So far, we have seemingly demonstrated an universal positive correlation between the \NC$_1$ and transferability. However, does the increase for the \NC$_1$ of learned features always lead to improved model transferability? To more comprehensively characterize the relationship between \NC$_1$ and transferability, we pre-train ResNet50 models on the Cifar-100 dataset using different levels of data augmentations and adversarial training \citep{madry2018towards, salman2020adversarially, deng2021adversarial} strength,\footnote{We use 5 levels of data augmentations, each level represents adding one additional type of augmentation, e.g., Level 1 means Normalization, level 2 means Normalization + RandomCrop, etc. For adversarial training strength, we follow the framework in \citet{madry2018towards} and consider 5 different attack sizes. Please refer to Appendix \ref{app:training_detail} for more details.} and then report the transfer accuracy of the pre-trained models on the Cifar-10 dataset. As shown in \Cref{fig:alg_adv_nc_fail}, we observe that the positive relationship between the \NC$_1$ on the source dataset and the transfer accuracy only holds up to a certain threshold.\footnote{The work \citet{kornblith2021why} studied the transferability based upon a notion called class separation, which is similar to our \NC$_1$\ metric. They concludes that there is a positive correlation between class separation and transfer accuracy. However, the work only studied the relationship within a limited range, for the cases that the class separation is large.
} If the \NC$_1$ metric is larger than a certain threshold, the transfer accuracy decreases as the \NC$_1$ increases.

We believe the reason behind the limitation is that the magnitude of $\mathcal{NC}_1$ is affected by two factors of the learned features: (\emph{i}) within class feature diversity and (\emph{ii}) between class discrimination. When the $\mathcal{NC}_1$ of is too large, the features lose the between-class discrimination, which results in poor transfer accuracy. An extreme example would be an untrained deep model with randomly initialized weights. Obviously, it possesses large \NC$_1$ with large feature diversity, but its features have poor between-class discrimination. Therefore, random features have poor transferability. To better predict the model transferability, we need more precise metrics for measuring both the within-class feature diversity and between-class discrimination, where the two could have a tradeoff between each other. We leave the investigation as future work.

%but it has 
%The answer is obviously \emph{no}. 



%So far, we have shown that models that are very collapsed on the source dataset have inferior transferability, which is aligned with the observation in \cite{hui2022limitations}. However, does this imply the truth of the opposite direction: models that are not collapsed on the source dataset will always transfer better? 


%Because the reason for the increase in $\mathcal{NC}_1$ could be either from the increase of feature diversity within each class or from the loss of discriminate power between classes.

%based upon the \NC$_1$ metric. 
%As shown in \Cref{fig:alg_adv_nc_fail}, 


 
% Our intuition is that the increase of variability will significant decrease the margin upon certain threshold.

% \qq{mixup data augmentation? learning stopping?}



 
%  lead to following claims
% \begin{itemize}[leftmargin=*]
%     \item \textbf{The usage of projection heads is not limited to contrastive losses.} Because the layer-wise progressive collapse is universal across the choice of training losses, the usage of projection head is not limited to contrastive losses nor self-supervised pre-training. As shown in our experiments in \Cref{fig:ce_nc_transfer}, we add different layers of projection heads for supervised pre-training models with the CE loss, which also substantially increase the transfer accuracy compared with that of no projection head. This suggests that the usage of projection for improving transferability can be universal.
%     \item \textbf{Projection heads promote feature diversity} Due to layer-wise progressive collapse, the additional projection layers prevent severe variability collapse of the encoder network. In our experiments, we add different number of projection layers (i.e., 1-3 layers) for model pre-training. \Cref{fig:ce_nc_transfer} (left) shows that more layers of projection head leads to better feature diversity of the encoder network, measured by $\mc {NC}_1$. However, as shown in \Cref{fig:ce_nc_transfer} (right), the trade-off is that projection head is decreasing the feature discrimination measured by $\mc {NC}_2$.
% \end{itemize}



%We argue that, by adding projection heads after the encoder, the features learned from the encoder become less collapse since the encoder is pushed away from the final layer and hence have superior representation power. As shown in \Cref{fig:ce_nc_transfer}, when no projection head is added, the within-class features are highly collapsed which results in a huge deficiency in the transfer accuracy. However, \Cref{fig:ce_nc_transfer} (Middle) also illustrates that feature diversity (i.e., larger $\mc {NC}_1$) is not the only deterministic factor that affect the transfer accuracy since the one-layer projection head model does not have the highest transfer accuracy. We find that the deterministic power of features also matters. \Cref{fig:ce_nc_transfer} (Right) shows that the features from the one-layer projection head model has the highest $\mc {NC}_2$ and thus the worst discriminative ability which sacrifices the representation power. Therefore, we believe there is an inherent trade-off between discrimination and diversity of learned features and the two properties mutually decide the representation ability of such features.


%Projection head refers to a linear or nonlinear multi-layer perception (MLP) module with dimension reduction, which is first introduced for contrastive learning \cite{chen2020simple, khosla2020supervised}.


%Projection head is a extensively used design choice in both supervised / self-supervised contrastive learning \cite{chen2020simple, khosla2020supervised}. Typically, a projection head $\mb g(\cdot)$ is a linear or MLP module that will be added after the encoder network and before applying the contrastive loss. But during inference, only the features from the encoder are considered and the projection head will be thrown away. 


%The intuition behind such design is that the projection head learns transformation-invariant representations so when applied to downstream tasks, such behavior may hinder the ability for effective transfer learning. The work \cite{chen2020simple} also empirically demonstrated that the features learned before projection head are superior in terms of classification accuracy. 

%In this work, we offer an additional view in the neuron collapse perspective and show that the beneficial of using projection heads is not only limited to contrastive losses, but also applicable to the CE loss. As previous result \cite{papyan2020traces} showed, neural collapse happens in deep networks in a cascading manner: the closer to the final layer, the severer the neural collapse.


 %   As shown in \Cref{fig:mlp_nc_transfer},      We train a $11$-layer MLP on Cifar-100 and conduct transfer learning on Cifar-10 using features from different layers. The results in \Cref{fig:mlp_nc_transfer} (Left) shows that features from latter layers are not superior in terms of transferability. On the other hand, the less collapsed features have better transfer learning performance, and we can observe a nearly linear relationship between $\mc {NC}_1$ and transfer learning accuracy from \Cref{fig:mlp_nc_transfer} (Right).
%     \item \textbf{Layers with larger feature diversity gaps between pre-trained and fine-tuned models are more important in fine-tuning.} When fine-tuning a pre-trained models on downstream tasks, not all layers are created of equal importance. In particular, after fine-tuning the network based upon the pretrained model, we find that layers with larger gaps of variability collapse between pretrained and fine-tuned models are more important to be fine-tuned. In our experiment in \Cref{fig:res18_finetune}, we pre-train a ResNet18 and fully fine-tune it on the downstream data, and then we compare the numerical rank of the output of each layer for both the pre-trained and fine-tuned network on the downstream data (denoted by the lines). In the meanwhile, for each layer we freeze all previous shallower layers and only fine-tune the layer and all deeper layers, and then we plot the transfer accuracy (denoted by the stars). As shown \Cref{fig:res18_finetune}, compared to fully fine-tuned network, we can see that the transfer accuracy starts to drop only when the gap of numerical rank between pre-trained and fine-tuned models becomes large. Here we use the numerical rank instead of $\mc {NC}_1$ becasue the feature dimension for the intermediate layers of ResNet is too large which makes the calculation of $\mc {NC}_1$ too expensive. Hence we use numerical rank as a surrogate. 
% \end{itemize}
% It is widely known that when fine-tuning a pretrained model on downstream tasks, fine-tuning more layers yield better performances \cite{kornblith2019better, zhang2019all}. However, fine-tuning the whole network could be very expensive for huge models. In contrast, as shown in our experiments here, using the \NC\ metrics as a guidance and being selective on few layers to be fine-tuned, we can substantially reduce computational cost for fine-tuning without sacrificing the performance.  As we observe, the general principle is that, for the pre-trained model to transfer on downstream tasks, we need the features of the pre-trained models to collapse on the downstream tasks at a similar level before or after fine-tuning.
% %achieve on-par performance wit
% \qq{adding some more discussion here to explain the implications on fine-tuning.}

%Interestingly, \Cref{fig:res18_finetune} shows that the increase in fine-tuning accuracy is not linear with the number of layers that are fine-tuned: the fine-tuning accuracy stays stable at the start, i.e., freeze the first few layers of the model and fine-tuning the others yield similar results as fine-tuning the entire model. To investigate this phenomenon, we calculated the $\widetilde{\text{rank}}$ (numerical rank) \cite{timor2022implicit} of each layer for the pretrained model and a fully fine-tuned model on the downstream Cifar-10 dataset. Surprisingly, we notice that there are minimal changes in $\widetilde{\text{rank}}$ for the beginning layers before/after fine-tuning which is also where the fine-tuning accuracies are stable. And when the changes in $\widetilde{\text{rank}}$ become more dramatic, we can also observe a seemingly drop in the fine-tuning accuracy. \xiao{what can we learn from this observation?} We also note another interesting phenomenon from \Cref{fig:res18_finetune}: the intrinsic dimensions of representations for different layers (approximated by $\widetilde{\text{rank}}$) shows a pattern of first increasing and then gradually decreasing. This observation is aligned with the work \cite{ansuini2019intrinsic}.

%\paragraph{\NC\ provides explanation for transfer learning using different layers.}
%The above analysis also casts doubt on the typical setting for conducting transfer learning: use all layers of a pretrained model up to the penultimate layer as a feature encoder and train a linear classifier for downstream tasks. The reason behind such design is that we believe features from latter layers of a model often contains more distilled information and hence are more powerful to transfer. But as shown in \cite{papyan2020traces}, features from latter layers are more collapsed and from the analysis above, we know collapsed features are often less transferable. Hence, in this section, we empirically examine the relationship between collapsing and transferability of different layers of a model. We train a $11$-layer MLP on Cifar-100 and conduct transfer learning on Cifar-10 using features from different layers. The results in \Cref{fig:mlp_nc_transfer} (Left) shows that features from latter layers are not superior in terms of transferability. On the other hand, the less collapsed features have better transfer learning performance, and we can observe a nearly linear relationship between $\mc {NC}_1$ and transfer learning accuracy from \Cref{fig:mlp_nc_transfer} (Right).

% %\paragraph{\NC\ provides guidance on model fine-tuning}
% %\begin{wrapfigure}[21]{r}{0.5\textwidth}
% %    \vspace{-0.1in}
% \begin{figure}
%     \centering
%     \includegraphics[width = 0.48\textwidth]{figs/res18_finetune.pdf}
%     \caption{\textbf{$\widetilde{\text{rank}}$ of input features for each layer and corresponding fine-tuning accuracy.} A ResNet18 model is pretrained using the Cifar-100 dataset and fine-tuned on downstream Cifar-10 dataset. $\widetilde{\text{rank}}$ is evaluated on the Cifar-10 dataset.}
%     \label{fig:res18_finetune}
% \end{figure}
% %\end{wrapfigure}

%\footnote{Numerical rank is an estimation of the true rank and is defined for for any matrix $\mb X$ as $\widetilde{\text{rank}} = ||\mb X||_F^2 / ||\mb X||_2^2$ \cite{timor2022implicit}.}
